Adaptive Kernel Kalman Filter

Sequential Bayesian filters in non-linear dynamic systems require the recursive estimation of the predictive and posterior distributions. This paper introduces a Bayesian filter called the adaptive kernel Kalman filter (AKKF). With this filter, the arbitrary predictive and posterior distributions of hidden states are approximated using the empirical kernel mean embeddings (KMEs) in reproducing kernel Hilbert spaces (RKHSs). In parallel with the KMEs, some particles, in the data space, are used to capture the properties of the dynamical system model. Specifically, particles are generated and updated in the data space, while the corresponding kernel weight mean vector and covariance matrix associated with the feature mappings of the particles are predicted and updated in the RKHSs based on the kernel Kalman rule (KKR). Simulation results are presented to confirm the improved performance of our approach with significantly reduced particle numbers, by comparing with the unscented Kalman filter (UKF), particle filter (PF) and Gaussian particle filter (GPF). For example, compared with the GPF, the proposed approach provides around 5% logarithmic mean square error (LMSE) tracking performance improvement in the bearing-only tracking (BOT) system when using 50 particles.

==> Adaptive Kernel Kalman Filter_Final/acronyms.tex <==
\acrodef{KME}{kernel mean embedding}
\acrodef{DSSM}{dynamic state-space model}
\acrodef{pdf}{probability density function}
\acrodef{EKF}{extended Kalman filter}
\acrodef{AKKF}{adaptive kernel Kalman filter}
\acrodef{KKR}{kernel Kalman rule}
\acrodef{GPF}{Gaussian particle filter}
\acrodef{RKHS}{reproducing kernel Hilbert space}
\acrodef{UKF}{unscented Kalman filter}
\acrodef{PF}{particle filter}
\acrodef{GPF}{Gaussian particle filter}
\acrodef{BOT}{bearing-only tracking}
\acrodef{KF}{Kalman filter}
\acrodef{KBR}{kernel Bayes' rule}
\acrodef{UNGM}{univariate nonstationary growth model}
\acrodef{MSE}{mean square error}
\acrodef{CV}{constant velocity}
\acrodef{LMSE}{logarithmic mean square error}
\acrodef{AWGN}{additive white Gaussian noise}
\acrodef{MC}{Monte Carlo}
\acrodef{CT}{coordinated turn}










